Neural Collaborative Filtering to Detect Anomalies in Human Semantic Trajectories

Human trajectory anomaly detection has become increasingly important across a wide range of applications, including security surveillance and public health. However, existing trajectory anomaly detection methods are primarily focused on vehicle-level traffic, while human-level trajectory anomaly detection remains under-explored. Since human trajectory data is often very sparse, machine learning methods have become the preferred approach for identifying complex patterns. However, concerns regarding potential biases and the robustness of these models have intensified the demand for more transparent and explainable alternatives. In response to these challenges, our research focuses on developing a lightweight anomaly detection model specifically designed to detect anomalies in human trajectories. We propose a Neural Collaborative Filtering approach to model and predict normal mobility. Our method is designed to model users' daily patterns of life without requiring prior knowledge, thereby enhancing performance in scenarios where data is sparse or incomplete, such as in cold start situations. Our algorithm consists of two main modules. The first is the collaborative filtering module, which applies collaborative filtering to model normal mobility of individual humans to places of interest. The second is the neural module, responsible for interpreting the complex spatio-temporal relationships inherent in human trajectory data. To validate our approach, we conducted extensive experiments using simulated and real-world datasets comparing to numerous state-of-the-art trajectory anomaly detection approaches.

==> content/baselines.tex <==
We compare with several unsupervised trajectory outlier detection methods, including three rule-based non-deep learning methods and two state-of-the-art deep learning methods:\\

%\textbf{DeepTEA} \cite{han2022deeptea} is a recently proposed deep learning framework designed for time-dependent trajectory outlier detection by capturing the dynamics of traffic patterns and the temporal dependencies of movements. It uses a combination of convolutional neural networks (CNNs) and recurrent neural networks (RNNs) to learn the normal patterns of trajectories over time. This approach allows DeepTEA to effectively identify outliers by comparing new trajectory data against learned patterns, taking into account both spatial and temporal characteristics, thus providing accurate and efficient online detection of anomalous trajectories.

==> content/droped_content.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=1.0\textwidth,center}
        \begin{tabular}{@{}lcccccccccccc@{}}
            \toprule
                                      & \multicolumn{4}{c}{ATL}     & \multicolumn{4}{c}{NOLA}        & \multicolumn{4}{c}{FVA}                                                                                                                                                      \\
            \cmidrule(lr){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13}
            Model                     & Top-10 Hits                 & Top-100 Hits\textsuperscript{*} & AP score                 & AUC score       & Top-10 Hits & Top-100 Hits & AP score        & AUC score       & Top-10 Hits & Top-100 Hits & AP score        & AUC score       \\
            \midrule
            OMPAD                     & 0                           & 7                               & 0.0571                   & 0.5257          & 2           & 10           & 0.0776          & 0.5968          & 0           & 4            & 0.0598          & 0.5322          \\
            MoNav-TT                  & 1                           & 5                               & 0.0893                   & 0.4863          & 1           & 3            & 0.0503          & 0.5026          & 0           & 0            & 0.0501          & 0.5014          \\
            TRAOD                     & 1                           & 10                              & 0.0582                   & 0.5018          & 0           & 4            & 0.0485          & 0.5011          & 0           & 7            & 0.0515          & 0.5090          \\
            DSVDD\textsuperscript{**} & 5                           & 36                              & 0.2601                   & 0.5835          & 9           & 28           & 0.2093          & 0.5829          & 5           & 26           & 0.2166          & 0.5995          \\
            DAE\textsuperscript{**}   & 3                           & 17                              & 0.0962                   & 0.5465          & 1           & 7            & 0.0648          & 0.5885          & 1           & 7            & 0.0569          & 0.5138          \\
            GM-VSAE                   & 4                           & 29                              & 0.1987                   & 0.5564          & 5           & 20           & 0.1786          & 0.5672          & 4           & 22           & 0.1534          & 0.5859          \\
            DeepTEA                   & 5                           & 26                              & 0.2008                   & 0.6012          & 5           & 26           & 0.2186          & 0.6395          & 5           & 30           & 0.2221          & 0.6182          \\
            \midrule
            TOD4Traj-MLP              & \textbf{10}                 & 34                              & 0.2782                   & 0.6824          & \textbf{10} & 41           & 0.3376          & 0.6985          & \textbf{10} & 32           & 0.2509          & 0.6561          \\
            TOD4Traj-RNN              & \textbf{10}                 & 32                              & 0.2780                   & 0.6233          & \textbf{10} & 27           & 0.2325          & 0.5940          & \textbf{10} & 27           & 0.2325          & 0.5940          \\
            TOD4Traj-CNN              & \textbf{10}                 & \textbf{42}                     & \textbf{0.3205}          & \textbf{0.7215} & \textbf{10} & \textbf{46}  & \textbf{0.3631} & \textbf{0.7185} & \textbf{10} & \textbf{40}  & \textbf{0.3151} & \textbf{0.6669} \\
            TOD4Traj-Former           & \textbf{10}                 & 34                              & 0.2436                   & 0.6735          & \textbf{10} & 34           & 0.2903          & 0.6970          & \textbf{10} & 33           & 0.2171          & 0.6628          \\
            \midrule
                                      & \multicolumn{4}{c}{GeoLife} & \multicolumn{4}{c}{ATL-Large}   & \multicolumn{4}{c}{BJNG}                                                                                                                                                     \\
            \cmidrule(lr){2-5} \cmidrule(l){6-9}\cmidrule(l){10-13}
            OMPAD                     & 1                           & 4                               & 0.1665                   & 0.1697          & 3           & 20           & 0.1461          & 0.6028          & 1           & 9            & 0.0704          & 0.5655          \\
            MoNav-TT                  & 0                           & 7                               & 0.2849                   & 0.3989          & 1           & 5            & 0.0893          & 0.4863          & 1           & 5            & 0.0893          & 0.4863          \\
            TRAOD                     & 4                           & 7                               & 0.1060                   & 0.5498          & 0           & 1            & 0.0030          & 0.4390          & 0           & 6            & 0.0553          & 0.5169          \\
            DSVDD\textsuperscript{**} & 7                           & 15                              & 0.6246                   & 0.7714          & 1           & 14           & 0.1010          & 0.4911          & 10          & 29           & 0.2155          & 0.5643          \\
            DAE\textsuperscript{**}   & 5                           & 12                              & 0.4627                   & 0.6234          & 4           & 19           & 0.1466          & 0.5641          & 0           & 10           & 0.0671          & 0.5568          \\
            GM-VSAE                   & 4                           & 13                              & 0.4892                   & 0.6034          & 2           & 12           & 0.1243          & 0.5482          & 4           & 16           & 0.1068          & 0.5479          \\
            DeepTEA                   & 6                           & 14                              & 0.5290                   & 0.7540          & 4           & 22           & 0.1752          & 0.6398          & 6           & 24           & 0.2084          & 0.5873          \\
            \midrule
            TOD4Traj-MLP              & \textbf{8}                  & \textbf{17}                     & \textbf{0.8512}          & \textbf{0.9397} & 4           & 28           & 0.2632          & 0.6737          & \textbf{10} & 34           & 0.2800          & 0.6587          \\
            TOD4Traj-RNN              & 7                           & 11                              & 0.6359                   & 0.7467          & 3           & 12           & 0.1310          & 0.5294          & \textbf{10} & 31           & 0.2573          & 0.6065          \\
            TOD4Traj-CNN              & 6                           & 16                              & 0.6756                   & 0.8542          & \textbf{10} & \textbf{40}  & \textbf{0.4572} & \textbf{0.7141} & \textbf{10} & \textbf{66}  & \textbf{0.4899} & \textbf{0.7513} \\
            TOD4Traj-Former           & 7                           & 16                              & 0.6283                   & 0.8889          & 8           & 27           & 0.2783          & 0.6852          & \textbf{10} & 33           & 0.2499          & 0.6219          \\
            \bottomrule
        \end{tabular}

    \end{adjustbox}
    \caption{Outlier detection performance for all datasets. The best performance for AP and AUC scores is highlighted for each dataset. \textsuperscript{*}We report Top-25 Hits instead of Top-100 for GeoLife dataset due to its size constraint. \textsuperscript{**}For implementation of comparison methods DSVDD and DAE, we only report the best performance of deep learning based competitive methods among the choice of four deep encoders (MLP, RNN, CNN and Transformer) for each dataset due to the limitation of the space.}\label{table:performance}
    \vspace{-0.3cm}
\end{table*}

==> content/related_works_old.tex <==
%Importance of outlier detection
In this section, we first introduce the fundamental definitions for Person-level trajectory outlier detection.

Next, we provide a comprehensive introduction to the collaborative filtering method, covering its algorithm, applications, and recent developments.

Following that, we summarize widely used outlier detection methods, both traditional and deep neural network (DNN) approaches, and highlight their limitations in the context of human-level trajectory outlier detection.

\subsection{Basic Concepts}
An outlier is commonly defined as a data point that is significantly different from the remaining data. Outliers are also referred to as abnormalities, discordants, deviants, or anomalies in the data mining and statistics literature~\cite{aggarwal2017introduction}.

Meanwhile, a spatial trajectory is a trace generated by a moving object in geographical spaces,usually represented by a series of chronologically ordered points~\cite{zheng2015trajectory}. 

Building upon the previous definitions, we define person-level human trajectories as the individual mobility of a person within a spatial area over a specific temporal period.

At each observation time, an agent reports their current location along with relevant contextual information such as acceleration, speed, and other pertinent metrics.

A human trajectory outlier, in this context, refers to a movement pattern at a specific period or location that significantly deviates from the individual's historical record or the movements of other individuals within the same group.


%In this context, a human trajectory outlier refers to a movement pattern at a specific time or location that significantly deviates from the individual’s historical record or the movements of other individuals within the same group.


\subsection{Outlier Detection Methodologies}
Over the past decades, a diverse array of outlier detection methods have been developed.
In this part, we will systematically classify these methods based on their training approaches.
Following that, we will categorize them into traditional and machine-learning driven methods.\textcolor{red}{[NEED CHANGE NO IDEA NOW]}


\subsubsection{Training approach}\textcolor{red}{[NEED CHANGE NO IDEA NOW]}
%\textbf{Training approach}:
The most widely used approach in outlier detection is \textit{no prior knowledge training}, often referred to as no-label training.

In this method, rare or unseen events within a scene are classified as abnormal.

The training dataset consists exclusively of normal activities, whereas the test dataset includes both normal and abnormal activities.

This allows the model to learn what constitutes normal behavior and flag any deviations during testing as potential outliers.

Liu et al.~\cite{liu2008isolation} proposed the Isolation Forest algorithm, which detects anomalies using binary trees.

Their idea hinges on the fact that outliers are a minority and exhibit attribute values significantly different from those of normal instances.

This method isolates anomalies by recursively partitioning the data into subsets.

When a forest of random trees collectively produces shorter path lengths for specific samples, those samples are considered anomalies.

Salvador and Chan~\cite{salvador2005learning} constructed an enhanced finite state automaton (FSA) for anomaly detection. Their model consists of three components: segmentation, rule generation (characterization), and state-transition logic.

An anomaly is detected when the FSA reaches a state with no outgoing edge that corresponds to the last symbol of the current sub-sequence.

Another widely used method is \textit{labeled dataset training}.

This approach utilizes a pre-labeled dataset with labels that indicate whether each data point is normal or abnormal.

Li et al. ~\cite{li2006motion} proposed a method to detect suspicious vessels based on motif feature extraction. A support vector machine (SVM) classifier is applied to these extracted features to identify anomalies.


Gao et al.~\cite{gao2002hmms} employed Hidden Markov Models (HMMs) to learn both normal and abnormal patterns of Unix processes.

They began by generating unique sequences of system calls, which were then used by the HMMs to classify patterns based on various window sizes and regions.
The model can be trained as a binary classifier, where any data point outside the normal class is considered an outlier.
Alternatively, it can be configured as a multi-class classifier, allowing the normal class to be divided into distinct categories through optimization ~\cite{yi2018speedup}.

This approach allows for a more nuanced classification of normal and abnormal data, enhancing the accuracy of detecting various types of normal behavior and potential anomalies.

The final approach, though less common, resembles online learning and requires a pre-classified dataset where the majority of the data are normal. This method, which involves \textit{learning from imbalanced data}, operates on the principle that negative inputs (abnormal data) are recognized as novel compared to positive inputs (normal data), which are more familiar due to their predominance in the training set.

It operates on the principle that negative inputs (abnormal data) are identified as novel compared to positive inputs (normal data), which are more familiar since they belong to the class used for training.


In the first phase, the model learns from positive instances only, establishing a baseline of normal behavior. In the second phase, it learns to differentiate between positive and negative instances of that concept, thereby identifying abnormalities.
The model can be incrementally tuned to enhance its accuracy as new data batches become available, ensuring it remains effective at detecting outliers even as underlying data patterns evolve. This continuous learning process allows the model to adapt to new trends and variations, maintaining its robustness and reliability over time ~\cite{japkowicz1995novelty,hodge2004survey}.

\subsubsection{Conventional and machine learning approaches}
Additionally, beyond classifying methods based on training set labels or the percentage of negative data, outlier detection methods can also be categorized into conventional and machine learning approaches. Conventional methods typically rely on statistical or rule-based techniques, while machine learning methods use data-driven algorithms to detect anomalies.

\textit{Statistical and probabilistic methods} are commonly used in conventional outlier detection. These methods rely on probability distributions, such as the Gaussian distribution, to identify data points that significantly deviate from the norm. By analyzing how data points fit within these distributions, these methods can detect anomalies that fall outside the expected range.



In detail, these methods are further divided into parametric and non-parametric approaches.

Parametric methods assume a specific distribution model for the data and estimate the model parameters based on the observed data.

In contrast, non-parametric methods do not assume any prior knowledge about the distribution model and instead use the data to determine the distribution directly.

Chen et al.~\cite{chen2009robust} proposed a probabilistic PCA (PPCA) with an expectation-maximization (EM) algorithm for maximum likelihood estimation of model parameters in the presence of missing data and introduced a contribution analysis method to identify which variables contribute to the most to the occurrence of outliers.

Yuen \& Mu~\cite{yuen2012novel} introduced a probabilistic method for parametric identification and outlier detection that quantifies the probability of a data point being an outlier.

Additionally, \textit{density-based methods} are also prevalent in the outlier detection domain. In these methods, anomalies are identified by assessing deviations in local density compared to the density of surrounding data points.

Breunig et al.~\cite{breunig2000lof} introduced the Local Outlier Factor (LOF), a method for quantifying how outlying a point is. LOF uses k-nearest neighbors and reachability distance to estimate local density. Points with significantly lower densities are identified as outliers.

Tang et al.~\cite{tang2017local} proposed a method for detecting outliers using local kernel density estimation (KDE), introducing the Relative Density-based Outlier Score (RDOS) to calculate the local outlier score of data points based on the density distribution estimated from their extended nearest neighbors.


Lastly, other approaches include \textit{clustering-based methods} and \textit{distance-based methods}.

Clustering-based methods categorize data based on similarity measures. Anomaly scores are computed by assessing how well subsequences align with the identified clusters, flagging data points that do not fit well within any cluster as anomalies.

Distance-based methods, on the other hand, focus on the concept of a data point's neighborhood, typically defined by its $k$ closest neighbors. Anomalies are identified based on the distance between a data point and its neighbors, with points that are significantly farther from their neighbors being considered outliers.

Chauhan \& Shukla ~\cite{chauhan2015review} evaluated various outlier detection techniques on data streams by applying different variations of the K-Means algorithm.

Thang \& Kim ~\cite{thang2011anomaly} proposed an improved DBSCAN algorithm, known as DBScan-MP, where each cluster may have different epsilon and minpts values, enhancing its adaptability and performance in identifying clusters and outliers.


Knorr \& Ng ~\cite{knox1998algorithms} were the first to introduce this concept. In distance-based outlier detection, a data point is considered an outlier if there are fewer than $k$ other points within a specified distance ($\delta$) of it in the dataset.

They also proposed two algorithms: the nested loop algorithm and the cell-based algorithm. These algorithms aim to reduce the computational complexity associated with finding nearest neighbors in large datasets.


\subsubsection{Machine Learning Methods}


Rather than relying solely on conventional methods, machine learning approaches have gained significant traction.

Recent advancements in machine learning have introduced promising solutions for outlier detection, utilizing sophisticated neural network architectures to improve the identification of anomalies.

These developments offer enhanced capabilities for detecting complex patterns and deviations that traditional methods might miss.

In machine learning methods, we further categorize approaches based on neural model structure.

Considering the data sparsity and outlier attributes, \textit{Graph Neural Networks (GNNs)}, which are designed to work with graph-structured data, are increasingly used in trajectory outlier detection.

GNNs leverage the inherent structure of the data to identify outliers that traditional methods might miss.

By capturing complex spatial patterns and adapting to the data's structure, GNNs enhance the ability to detect anomalies effectively. ~\cite{sahili2023spatio}

Recently, there has been a significant advancement in GNN:
Goodge et al.~\cite{goodge2022lunar} proposed LUNAR which utilizes information from a node's nearest neighbors to identify anomalies.

Du et al. ~\cite{du2022graph}proposed an autoencoder-based unsupervised outlier detection, their GNN models are trained to reconstruct graph structure after aggregating neighboring feature values.

Deviations from the reconstruction can indicate outliers.

Zheng et al.\cite{zheng2019addgraph} introduced AddGraph, which combines an extended temporal GCN with an attention-based GRU to detect anomalies in dynamic graphs. It captures node and edge information, updating node embeddings and hidden states at each time step. Anomaly scores are assigned to edges based on the associated nodes.

Another category of deep learning models, aside from GNNs, includes various neural network approaches that treat the trajectory as a series to learn complex patterns and identify anomalies known as \textit{series learning models}.

These methods, including Recurrent Neural Networks (RNNs) and Long Short-Term Memory (LSTM) networks, are particularly effective for analyzing sequential or temporal data.

Their ability to capture long-term dependencies and patterns within the data makes them highly suitable for tasks such as time-series forecasting, anomaly detection, and sequence modeling.

Niu et al.~\cite{niu2018alstm}introduce an adaptive LSTM that utilizes temporal continuity in sequential data. By incorporating a mask gate and maintaining span, this LSTM can update memory adaptively based on changes in the sequence input at each time step.

Lu et al.~\cite{lu2017unsupervised}propose Unsupervised Sequential Outlier Detection with Deep Architecture (UODA), which combines autoencoders for density-based outlier detection, and deep RNNs for context learning.


\subsection{Collaborative Filtering}

Collaborative Filtering (CF), first introduced in the 1990s~\cite{10.1145/138859.138867}, is a widely used technique in recommendation systems. Originally, CF involved users collaborating to filter information by recording their reactions to documents they read, allowing others to access these reactions.

As a popular recommendation model, Collaborative Filtering utilizes ratings or other forms of user feedback to identify shared preferences among users. It then provides personalized recommendations based on these similarities, without requiring external information about the items or users.

Collaborative Filtering employs two main techniques: the neighborhood approach and latent factor models.
~\cite{korenAdvancesCollaborativeFiltering2022}.

The neighborhood approach models a user's preference for an item based on their ratings of similar items, while latent factor models utilize a shared latent factor space between items and users to explain ratings.

Nowadays, by leveraging advanced techniques such as matrix factorization ~\cite{bokde2015matrix}, singular value decomposition ~\cite{paterek2007improving} and integration of deep learning~\cite{wei2017collaborative,bobadilla2020deep,he2017neural} have further enhanced the accuracy and scalability of Collaborative Filtering models.





==> meta/ccs.tex <==


%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%


\begin{CCSXML}

    <ccs2012>
    <concept>
    <concept_id>10002951.10003227.10003236.10003237</concept_id>
    <concept_desc>Information systems~Geographic information systems</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    <concept>
    <concept_id>10002951.10003227.10003236.10003101</concept_id>
    <concept_desc>Information systems~Location based services</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Geographic information systems}
\ccsdesc[500]{Information systems~Location based services}

